Temporal Variability in Implicit Online Learning

In the setting of online learning, Implicit algorithms turn out to be highly successful from a practical standpoint. However, the tightest regret analyses only show marginal improvements over Online Mirror Descent. In this work, we shed light on this behavior carrying out a careful regret analysis. We prove a novel static regret bound that depends on the temporal variability of the sequence of loss functions, a quantity which is often encountered when considering dynamic competitors. We show, for example, that the regret can be constant if the temporal variability is constant and the learning rate is tuned appropriately, without the need of smooth losses. Moreover, we present an adaptive algorithm that achieves this regret bound without prior knowledge of the temporal variability and prove a matching lower bound. Finally, we validate our theoretical findings on classification and regression datasets.

==> doubling.tex <==
\section{Doubling Trick}
\label{sec:doubling}

In this section, we present a doubling trick strategy to tune the learning rate in IOMD.

First, we overload the notation by introducing $\delta_t^i$ defined as follows
\begin{equation}
\label{eq:delta_t_doubling}
    \delta_t^i \triangleq \ell_t(\bx_t) - \ell_t(\bx_{t+1}') - \frac{1}{\eta_i} B_\psi(\bx_{t+1}', \bx_t)~.
\end{equation}
The algorithm works as follows: we set a learning rate $\eta_i$, IOMD and monitor the sum $ \sum_t \delta_t(\eta_i) / \eta_i $ until it reaches $ 2^i L^2 $. Once this happens, we restart the algorithm doubling the threshold and halving the learning rate---see \cref{algo:implicit_MD}.

\begin{algorithm}[t]
\caption{IOMD with doubling trick}
\label{algo:implicit_MD}
\begin{algorithmic}[1]
{
\REQUIRE{Non-empty closed convex set $V \subset X \subset \mathbb{R}^d $, distance generating function $\psi: \mathbb{R}^d \rightarrow \mathbb{R}$, Lipschitz constant $L > 0$, $1>0$}
\STATE{Initialize: $i = 0$, $ S_0 = 0 $, $\bx_1 = \boldsymbol{0}, \eta_0=\frac{1}{L}$}
\FOR{$t=1,\dots,T$}
\STATE{Output $\bx_t$}
\STATE{Receive $\ell_t: \mathbb{R}^d \rightarrow (-\infty, + \infty]$ and pay $\ell_t(\bx_t)$}
\STATE{$\bx'_{t+1} = \arg\min_{\bx \in V} \  B_{\psi}(\bx, \bx_t) + \eta_i \ell_t(\bx) $}
\STATE{$S_i \leftarrow S_i + \ell_t(\bx_t) + \ell_t(\bx'_{t+1}) - \frac{1}{\eta_i} B_\psi(\bx_t, \bx'_{t+1})$}
\IF{$S_i \geq \eta_i L^2 2^i$}
\STATE{$i = i + 1$}
\STATE{Update $\eta_i = \frac{1}{L\sqrt{2^i}}$}
\STATE{$S_i = 0$}
\STATE{$\bx_{t+1} = \boldsymbol{0}$}
\ELSE
\STATE{$\bx_{t+1} = \bx'_{t+1}$}
\ENDIF
\ENDFOR
}
\end{algorithmic}
\end{algorithm}

For the analysis, denote by $t_i$ the index of the first round of epoch $i$. Also, $N$ is the total number of epochs and $t_{N+1}:=T+1$.
We first show that the total number of epochs is logarithmic in a quantity $\Delta_T$ which we define for the sake of the analysis. 
\begin{lemma}
\label{lemma:max_epoch}
Let $t_i$ be the first time-step of epoch $i$, with $t_0 = 1$. Suppose \cref{algo:implicit_MD} is run for a total of $N$ epochs. Let $\Delta_T$ be defined as 
\begin{equation}
\label{eq:sum_delta_t}
    \Delta_T \triangleq \sum_{i=0}^N \sum_{t=t_i}^{t_{i+1}-1} \frac{\delta_t(\eta_i)}{\eta_i}~.
\end{equation}
Then, we have that total number of epochs $N$ is bounded as $N \leq \log_2 \left( \frac{\Delta_T}{L^2} + 1 \right)$.
\end{lemma}
\begin{proof}
Using the notation introduced, we have that $\delta_{t_{i+1}-1}(\eta_i)$ is the term which causes the restart in epoch $i$. Therefore, the following holds
\begin{equation}
\label{eq:boundepoch}
\sum_{t=t_i}^{t_{i+1}-1} \frac{\delta_t(\eta_i)}{\eta_i}
\leq L^2\left(2^i + \frac{1}{2}\right),
\end{equation}
since from Lemma~\ref{lemma:failsafe} the last term in epoch $i$ is such that $\tfrac{d_{t_{i+1}-1}(\eta_i)}{\eta_i} \leq \tfrac{L^2}{2}$.

Note that the sum of the $L^2 2^i$ terms in the first $N-1$ epochs is less or equal than the final sum $ \Delta_T$. 
Using the fact that $\sum_{i=0}^{N-1} a^i = \frac{a^N - 1}{a - 1}$, we have
\begin{equation*}
    \sum_{i=0}^{N-1} 2^i L^2 = L^2 (2^N - 1) \leq \sum_{i=0}^N \sum_{t=t_i}^{t_{i+1}-1} \frac{\delta_t(\eta_i)}{\eta_i} = \Delta_T,
\end{equation*}
which yields the desired result.
\end{proof}

\begin{figure}[h!]
    \centering
    \begin{tikzpicture}
    \draw[thick,-] (0,0) -- (8,0) node[anchor=north west] {};
    \draw[dashed,->] (8,0) -- (13,0) node[anchor=north west] {$ \delta_t / \eta_i $ "axis"};
    \node [anchor=south] (zero) at (0,0) {0};
    \draw (0 cm,1.5pt) -- (0 cm,-1.5pt);
    \node [anchor=south] (one) at (1, 0) {1};
    \draw (1 cm,1.5pt) -- (1 cm,-1.5pt);
    \node [anchor=south] (two) at (3, 0) {2};
    \draw (3 cm,1.5pt) -- (3 cm,-1.5pt);
    \node [anchor=south] (three) at (7, 0) {3};
    \draw (7 cm,1.5pt) -- (7 cm,-1.5pt);
    \node [anchor=south] (end) at (8, 0) {$\Delta_T$};
    \draw (8 cm,1.5pt) -- (8 cm,-1.5pt);
    \draw [
    thick,
    decoration={
        brace,
        mirror,
        raise=0.5cm
    },
    decorate
    ] (zero) -- (one)
    node [pos=0.5,anchor=north,yshift=-0.55cm] {$L^22^0$};
    \draw [
    thick,
    decoration={
        brace,
        mirror,
        raise=0.5cm
    },
    decorate
    ] (one) -- (two)
    node [pos=0.5,anchor=north,yshift=-0.55cm] {$L^2 2^1$};
    \draw [
    thick,
    decoration={
        brace,
        mirror,
        raise=0.5cm
    },
    decorate
    ] (two) -- (three)
    node [pos=0.5,anchor=north,yshift=-0.55cm] {$L^2 2^2  $};
    \draw [
    thick,
    decoration={
        brace,
        raise=0.3cm
    },
    decorate
    ] (two) -- (three)
    node [pos=0.5,anchor=south,yshift=+0.55cm] {$ \leq \sum_{t=t_2}^{t_3-1} \frac{\delta_t(\eta_2)}{\eta_2} \leq L^2\left(2^2 + \frac{1}{2}\right) $};
\end{tikzpicture}
    \caption{Doubling trick illustrated.}
    \label{fig:doubling_trick}
\end{figure}

We can now analyze the regret incurred by the algorithm. Each epoch is bounded individually. The final regret bound is given by the sum of the individual contributions over all the epochs. 

\begin{theorem} \label{thm:regret_doubling}
Assume the losses $\ell_t(\bx)$ to be $L$-Lipschitz, for all $t=1, \ldots, T$ and $ \psi $ to be $1$-strongly convex w.r.t. $\| \cdot \|$. Let $\delta_t$ be defined as in \cref{eq:delta_t}. Then, for any $\bu \in \mathbb{R}^d$ the regret of \cref{algo:implicit_MD} after $T$ rounds is bounded as
\begin{equation} \label{eq:intermediate}
    R_T(\bu)
    \leq c \left(B_\psi(\bu, \boldsymbol{0}) + 1 \right)\sqrt{\sum_{i=0}^N \sum_{t=t_i}^{t_{i+1} - 1} \frac{\delta_t(\eta_i)}{\eta_i} + L^2} + c\frac{L}{2},
\end{equation}
where $c = \frac{\sqrt2}{\sqrt2 - 1}$.

Furthermore, using \cref{lemma:failsafe} we have that
\begin{equation} \label{bound:sqrtT}
R_T(\bu) 
\leq c L \left(B_\psi(\bu, \boldsymbol{0}) + 1 \right)\sqrt{T+1} + c\frac{L}{2}~.
\end{equation}
\end{theorem}
\begin{proof}
Let's first define $R_i(\bu)$ as the regret during epoch $i$,
\begin{equation*}
    R_i(\bu) = \sum_{t=t_i}^{t_{i+1}-1} (\ell_t(\bx_t) - \ell_t(\bu))~.
\end{equation*}
Using \cref{eq:base_constrained} with $\eta_t = \eta_i$ for $t \in [t_i, \ldots, t_{i+1}-1]$, we have that $R_i(\bu)$ is bounded as follows
\begin{align}
    R_i(\bu) 
    &\leq \frac{B_\psi(\bu, \bx_{t_i})}{\eta_i} + \sum_{t=t_i}^{t_{i+1}-1} \Big[ \ell_t(\bx_t) - \ell_t(\bx'_{t+1}) - \frac{1}{\eta_i} B_\psi(\bx'_{t+1}, \bx_t) \Big] \nonumber \\
    &\leq \frac{B_\psi(\bu, \bx_{t_i})}{\eta_i} + \sum_{t=t_i}^{t_{i+1}-1} \delta_t(\eta_i) 
    = \frac{B_\psi(\bu, \boldsymbol{0})}{\eta_i} + \sum_{t=t_i}^{t_{i+1}-1} \delta_t(\eta_i)~. \label{eq:regret_one_phase}
\end{align}

We can now write the final regret bound by summing $R_i(\bu)$ over all the epochs $i=1, \ldots, N$. \begin{align*}
    R_T(\bu) & = \sum_{i=0}^N R_i(\bu) \\
    & \leq \sum_{i=0}^N \left[ \frac{B_\psi(\bu, \boldsymbol{0})}{\eta_i} + \sum_{t=t_i}^{t_{i+1} - 1} \delta_t(\eta_i) \right] \\
    & \leq \sum_{i=0}^N \left[ \frac{B_\psi(\bu, \boldsymbol{0})}{\eta_i} + \eta_i L^2\left( 2^i + \frac{1}{2}\right) \right] & \textup{see \cref{eq:boundepoch}} \\
    & = L\left(B_\psi(\bu, \boldsymbol{0})+1\right) \sum_{i=0}^N \sqrt{2^i} + \frac{L}{2}\sum_{i=0}^N \frac{1}{\sqrt{2^i}} & \left(\eta_i = \frac{1}{L \sqrt{2^i}}\right)  \\
    & \leq \left(B_\psi(\bu, \boldsymbol{0})+1\right) L \frac{2^{\frac{N + 1}{2}} - 1 }{\sqrt{2} - 1} + \frac{ L\sqrt{2}}{2(\sqrt{2}-1)}&  \left(\sum_{i=0}^{N-1} a^i = \frac{a^N - 1}{a - 1}\right) \\
    & < \left(B_\psi(\bu, \boldsymbol{0})+1\right) \frac{L}{ \sqrt{2} - 1} 2^{\frac12 \log_2\left(\frac{\Delta_T}{L^2} + 1\right) + \frac12} + \frac{L\sqrt{2}}{2(\sqrt{2}-1)} \\
    & = \left(B_\psi(\bu, \boldsymbol{0})+1\right) \frac{\sqrt2}{\sqrt{2} - 1} L \sqrt{
    \frac{\Delta_T + L^2}{L^2}} + \frac{L\sqrt{2}}{2(\sqrt{2}-1)} \\
    & = c \left(B_\psi(\bu, \boldsymbol{0})+1\right) \sqrt{\Delta_T + L^2} + c \frac{L}{2},
\end{align*}
where in the last step we used the definition of $c$. Now, using the definition of $\Delta_T$ we get the bound in \cref{eq:intermediate}.

Furthermore, using \cref{lemma:failsafe} and the assumption on the losses to be $L$-Lipschitz, we get
\begin{align*}
    \Delta_T = \sum_{i=0}^N \sum_{t=t_i}^{t_{i+1} - 1} \frac{\delta_t(\eta_i)}{\eta_i} \leq \sum_{i=0}^N \sum_{t =t_i}^{t_{i+1} - 1} \frac{L^2}{2} = \frac{L^2}{2} T,
\end{align*}
substituting back the above result in \cref{eq:intermediate} gives the bound in \cref{bound:sqrtT}.
\end{proof}


\subsection{Fixed Losses}

If the losses are all equal, i.e. $\ell_t(\bx) = \ell(\bx)$ for all $t = 1, \ldots, T$, from \cref{thm:regret_doubling} and \cref{eq:intermediate} we get
\[
R_T(\bu) 
= \mathcal{O} \left( \sqrt{\sum_{i=0}^N \frac{1}{\eta_i} \left[ \ell(\bx_{t_i}) - \ell(\bx_{t_{i+1}}) - \frac{1}{\eta_i} \sum_{t=t_i}^{t_{i+1} - 1} B_\psi(\bx_{t+1}, \bx_t) \right] + L^2 } \right)~.
\]
However, note that with fixed losses the sum of the $\delta_t$ terms should not increase over time and the algorithm should always stay in the first epoch, so that the bound ideally would be
\begin{equation*}
    R_T(\bu) = \mathcal{O} \left( \sqrt{\frac{1}{\eta_0} \ell(\bx_1) + L^2} \right) = \mathcal{O} \left( \sqrt{L \left(\ell(\bx_1) + L \right)} \right)~.
\end{equation*}
This might not be entirely true: the algorithm will stay in the same phase depending on the first loss of the epoch $i$, $\ell(\bx_{t_i})$, as long as the condition $ \delta_t(\eta_i) / \eta_i \leq 2^i L^2$ is satisfied. But it can happen that the condition gets violated on the very first loss: in this case the algorithm might keep restarting until the condition will not be violated anymore. 
The next lemma establishes that this never happens and the algorithm always stays in the first epoch.
\begin{lemma} \label{lemma:restarts}
Assume the losses over time are fixed, i.e. $\ell_t(\bx) = \ell(\bx)$ for all $t = 1, \ldots, T $ and $\psi(\bx)$ be $1$-strongly convex w.r.t $\| \cdot \|$. Then, \cref{algo:implicit_MD} will always stay in the first epoch, i.e., $N=0$.
\end{lemma}
\begin{proof}
In order to not have a restart, we need $ \delta_t(\eta_i) \leq \eta_i L^2 2^i $, which translates to
\[
    \ell(\bx_t) - \ell(\bx'_{t+1})
    \leq L\sqrt{2^i}\left(B_\psi(\bx'_{t+1}, \bx_t)+1\right)~.
\]
From the inequality above, we have a reset iff
\begin{align*}
    i 
    & \leq 2 \log_2 \frac{\ell(\bx_t) - \ell(\bx'_{t+1}) }{L\left( B_\psi(\bx'_{t+1}, \bx_t)+1\right)} 
    \leq 2 \log_2 \frac{L \| \bx_t - \bx'_{t+1} \|}{L\left(1 + \frac{1}{2} \| \bx'_{t+1} - \bx_t \|^2 \right)} \\
    & = 2 \log_2 \frac{2 \| \bx'_{t+1} - \bx_t \| \bm}{ 2 + \| \bx'_{t+1} - \bx_t \|^2 },
\end{align*}
where the second inequality derives from the Lipschitzness of the losses and by lower bounding the Bregman divergence with \cref{eq:bregman_strongly_convex}. Now, let $f(y) = \frac{2 y}{2 + y^2}$, with $y \geq 0 $. We have that $ \lim_{y \rightarrow +\infty} f(y) = 0 $ and $ f(0) = 0 $. Furthermore, if we take the derivative and set it to 0, we see that $f(y)$ has a maximum in $ y = \sqrt{2} $. Hence, we have
\[
i
\leq 2 \log_2 \frac{2 \| \bx'_{t+1} - \bx_t \| \bm}{ 2 + \| \bx'_{t+1} - \bx_t \|^2 }
\leq 2 \log_2 \frac{\sqrt{2}}{2} = -1~.
\]
Therefore, if $i > -1$ then we will not double the learning rate. Note that this is always verified and we can conclude that $ N = 0 $.
\end{proof}

We are now ready to bound the regret in the case the losses over time are fixed. 
\begin{theorem}
Denote $\bg_t \in \partial \ell(\bx_t) $, $\bg_{\boldsymbol{0}} \in \partial \ell(\boldsymbol{0}) $ and assume $ \| \bg_t \|_\star \leq L $ for all $t=1, \ldots, T$. Then, under the assumptions of \cref{lemma:restarts} the regret of \cref{algo:implicit_MD} is bounded as
\begin{equation} \label{eq:fixed_losses_bound}
    R_T(\bu) 
    \leq L B_\psi(\bu, \bm{0}) + \ell(\bm{0}) - \ell(\bx_T)~.
\end{equation}
\end{theorem}
\begin{proof}
From \cref{eq:regret_one_phase} and the fact that we only have one epoch thanks to \cref{lemma:restarts}, we have that
\begin{align*}
    R_T(\bu) = R_0(\bu) & \leq \frac{B_\psi(\bu, \bx_1)}{\eta_0} + \sum_{t=1}^T \delta_t(\eta_0) \\
        & = \frac{B_\psi(\bu, \bx_1)}{\eta_0} + \sum_{t=1}^T \left[ \ell(\bx_t) - \ell(\bx_{t+1}) - \frac{B_\psi(\bx_{t+1}, \bx_t)}{\eta_0} \right] \\
        & \leq \frac{B_\psi(\bu, \bm{0})}{\eta_0}  + \ell(\bx_1) - \ell(\bx_T) \\
        & = L B_\psi(\bu, \bm{0}) + \ell(\bm{0}) - \ell(\bx_T)
\end{align*}

\iffalse

Again, we write the final regret as a sum of individual contributions over epochs. We have
\[
R_T(\bu) 
= \sum_{i=0}^{N-1} R_i(\bu) + R_N(\bu) 
= \underbrace{\sum_{t=1}^{t_1-1} (\ell(\bx_{t})- \ell(\bu))}_{\textup{(a)}} + \underbrace{\sum_{t=t_1}^T (\ell(\bx_{t}) - \ell(\bu))}_{\textup{(b)}}~.
\]
We analyze the contribution of the two terms above separately. From \cref{eq:boundepoch}, term (a) is upper bounded by
\[
\sum_{t=1}^{t_1} \left(\ell(\bx_{t})- \ell(\bu)\right)
\leq \frac{B_\psi(\bu,\boldsymbol{0})}{\eta_0} + \eta_0 L^2 \left(1+\frac{1}{2}\right)
= L\left(\frac{B_\psi(\boldsymbol{0},\bu)}{1} + \frac{31}{2} \right)~.
\]
On the other hand, for (b) from \cref{eq:base_constrained} we get
\begin{align*}
\sum_{t=t_1}^T (\ell(\bx_{t}) - \ell(\bu))
& \leq \frac{B_\psi(\bu, \bx_{t_1})}{\eta_1} + \sum_{t=t_N}^T \left[ \ell(\bx_t) - \ell(\bx'_{t+1}) - \frac{1}{\eta_1} B_\psi(\bx'_{t+1}, \bx_t) \right] \\
& =\frac{B_\psi(\bu, \boldsymbol{0})}{\eta_1} + \sum_{t=t_N}^T \left[ \ell(\bx_t) - \ell(\bx_{t+1}) - \frac{1}{\eta_1} B_\psi(\bx_{t+1}, \bx_t) \right] \\
& = \frac{B_\psi(\bu, \boldsymbol{0})}{\eta_1} + \ell(\boldsymbol{0}) - \ell(\bx_{T+1}) - \frac{1}{\eta_1} \sum_{t=t_N}^T B_\psi(\bx_{t+1}, \bx_t) \\
& \leq \frac{B_\psi(\bu, \boldsymbol{0})}{\eta_1} + \ell(\boldsymbol{0}) - \ell(\bx_{T+1}) \\
& = L \sqrt{2}\frac{B_\psi(\bu, \boldsymbol{0})}{1 } + \ell(\boldsymbol{0}) - \ell(\bx_{T+1})~.
\end{align*}

Putting (a) and (b) together, we get the stated bound.

\fi


\end{proof}


\section{Proofs}
\label{sec:proofs}


\begin{proof}[Proof of \Cref{theo:properties}]
From \cref{eq:loss_better} and the update in \cref{eq:constrained_update}, we immediately get the following inequality
\begin{equation*}
\eta_t \ell_t(\bx_{t+1}) 
\leq \eta_t \ell_t(\bx_{t+1}) + B_\psi(\bx_{t+1}, \bx_t) 
\leq \eta_t \ell_t(\bx_t) + B_{\psi}(\bx_t, \bx_t) 
= \eta_t \ell_t (\bx_t),
\end{equation*}
that implies that value of the loss $\ell_t$ in $\bx_{t+1}$ is not bigger than the one in $\bx_t$. 

\cref{eq:optimality} is simply the first-order optimality condition for $\bx_{t+1}$.

For \cref{eq:prop3}, from the convexity of $\ell_t$ we have
\begin{align*}
\ell_t(\bx_{t+1}) &\geq \ell_t(\bx_t)+\langle \bg_t, \bx_{t+1}-\bx_{t}\rangle,\\
\ell_t(\bx_{t}) &\geq \ell_t(\bx_{t+1})+\langle \bg'_t, \bx_{t}-\bx_{t+1}\rangle~.
\end{align*}
Summing both inequalities, we get the desired result.
\end{proof}


\begin{proof}[Proof of \Cref{lemma:master_lemma}]
From \cref{eq:optimality}, we have that
\begin{align*}
\eta_t(\ell_t(\bx_{t+1}) - \ell_t(\bu))
& \leq \langle \eta_t \bg_t', \bx_{t+1} - \bu \rangle 
\leq  \langle \nabla \psi(\bx_t) - \nabla \psi(\bx_{t+1}), \bx_{t+1} - \bu \rangle \\
& = B_\psi (\bu, \bx_t ) - B_\psi(\bu, \bx_{t+1}) - B_\psi(\bx_{t+1}, \bx_t ) ~.
\end{align*}
Dividing by $\eta_t$ and summing over $t=1, \ldots, T$ yields the result in \cref{eq:constrained_partial_1}.

For the second part observe that
\begin{align*}
\sum_{t=1}^T \frac{ B_\psi(\bu, \bx_t) - B_\psi(\bu, \bx_{t+1})}{\eta_t} 
& \leq \frac{D^2}{\eta_1} + D^2 \sum_{t=2}^T \left( \frac{1}{\eta_{t}} - \frac{1}{\eta_{t-1}} \right)
= \frac{D^2}{\eta_T} ~. \qedhere
\end{align*}
\end{proof}



\begin{proof}[Proof of \Cref{lemma:adahedge}]
From the assumptions, we have that $\Delta_{t+1} \le \Delta_t + \min \left\{ b a_t, \ c a_t^2/(2\Delta_t) \right\}$, for any $t \ge 1$. Also, observe that
\[
\Delta_{T+1}^2 
= \sum_{t=1}^T \Delta_{t+1}^2 - \Delta_{t}^2 
= \sum_{t=1}^T \left[\underbrace{(\Delta_{t+1} - \Delta_t)^2}_{\textup{(a)}} + \underbrace{2 (\Delta_{t+1} - \Delta_t) \Delta_t}_{\textup{(b)}}\right]~.
\]
We bound (a) and (b) separately. For (a), from the assumption on the recurrence and using the first term in the minimum we have that $(\Delta_{t+1} - \Delta_t)^2 \leq b^2 a_t^2 $. On the other hand, for (b) using the second term in the minimum in the recurrence we get $2(\Delta_{t+1} - \Delta_t) \Delta_t \leq c a_t^2 $. Putting together the results we have that $\Delta_{T+1}^2 \leq (b^2 + c) \sum_{t=1}^T a_t^2$ and the lemma follows.
\end{proof}


\section{Formulas}
\label{sec:formulas}

First, let's mention the update rules for IOMD with $V=\R^d$ for hinge loss, absolute loss, and square loss respectively \cite[see, e.g.,][]{CrammerDKSSS06,KulisB10}.
\begin{align*}
\bx_{t+1} &= \bx_t + \min\left(\eta_t, \frac{\max(1-y_t \langle \bz_t, \bx_t\rangle,0)}{\|\bz_t\|^2}\right) y_t \bz_t,\\
\bx_{t+1} &= \bx_t - \min\left(\eta_t, \frac{|\langle \bz_t, \bx_t\rangle-y_t|}{\|\bz_t\|^2}\right) \bz_t,\\
\bx_{t+1} &= \bx_t - \eta_t \frac{(\langle \bz_t, \bx_t\rangle-y_t) \bz_t}{1+ \eta \|\bz_t\|_2^2}~.
\end{align*}

Now let's consider the case that $V=\{\bx: \|\bx\|_2\leq D/2\}$. In this case it is easy to see that the update becomes
\[
\bx_{t+1} = \bx_t - \eta_t \bg'_t - \alpha \bx_{t+1},
\]
where $\bg_t' \in \partial \ell_t(\bx_{t+1})$, $ \alpha \bx_{t+1} \in \partial i_V(\bx_{t+1})$ and $\alpha\geq0$.
Hence, we have that
\[
\bx_{t+1} = \frac{\bx_t}{\alpha+1} - \frac{\eta_t}{\alpha+1} \bg'_t~.
\]
This implies that we can take the previous formulas and substitute $\frac{\bx_t}{\alpha+1}$ to $\bx_t$ and $\frac{\eta_t}{\alpha+1}$ to $\eta$.
Then, the optimal $\alpha \geq 0$ is the smallest one that gives $\|\bx_{t+1}\| \leq D/2$. Note that this is a 1-dimensional problem that can be easily solved numerically.

